Do You Have the Right Scissors? Tailoring Pre-trained Language Models via Monte-Carlo Methods

It has been a common approach to pre-train a language model on a large corpus and fine-tune it on task-specific data. In practice, we observe that fine-tuning a pre-trained model on a small dataset may lead to over- and/or under-estimation problem. In this paper, we propose MC-Tailor, a novel method to alleviate the above issue in text generation tasks by truncating and transferring the probability mass from over-estimated regions to under-estimated ones. Experiments on a variety of text generation datasets show that MC-Tailor consistently and significantly outperforms the fine-tuning approach. Our code is available at this url.

==> 040analysis.tex <==
In this part, we give a thorough analysis of why finetuning is not enough for restricting large open domain models to small domains. 
\subsection{Phenomenon}
We finetune the GPT-2 on training data, and save the model with the lowest ppl on evalation data. Table~\ref{} is some examples of real data and generated ones. We find that a large proportion of generated samples are not in the same style as training data. We also use a CNN based classfier to quantify the difference between real and generated samples. It turns out that the classfier achieves 90\% accuracy in distinguishing between real and generated samples.

The finetuned GPT-2 has not fully adapted to the style in training samples. So it is a natural idea to continue training it until domain specific information is well learned.
However, since we has already selected the model with the lowest ppl, continuing training will lead to increased ppl. As indicated in Table~\ref{}, rev\_ppl will also not get better after the ppl has hit the lowest value.
\subsection{Analysis}
To explain why these seemingly contradictory phenomena happen, we need to dig deeper at the finetuning process. 
Gpt-2 is a well trained language model, which learns patterns of plausible sentences. There are different levels of patterns, from coarse to fine. Coarse patterns includes general regulation of sentences, for example, adjectives are usually followed by nouns. Fine grained patterns describe some specific knowledge. For example, in a generation task where the previous words are 'Trump is the president of', the next word should be 'USA' or 'America'.

We formulate the probability of a sentence $x \propto \sum_{i} \alpha_{i}M(x, Pattern_i)$. $M(x, Pattern_i)$ is a measure of whether x comply pattern $i$ and $\alpha_{i}$ is the relative importance of pattern $i$. When training a language model from scratch, the language model learns new patterns and adjust the corresponding $\alpha$ simultaneously. But things are much simpler when it comes to finetuning an open domain model, such as GPT-2, to a specific domain. The most patterns in the small domain is already learned by the large model. As a result, we mainly need to tune the importance factor. 
%Add an example of tuning \alpha

We assume that $Pattern_i$ for $i \in Pa_d$ is the correct pattern of domain $d$. So the aim of finetuning is to raise $\alpha_i$ for $i \in Pa_d$. However, in the case of data deficiency, the weight of a single training sample is not neglectable. Even though a pattern only appears once, learning this pattern can lower training loss. We use $Pa_{train}$ to denote all patterns in the training set, so $Pa_{train}-Pa_d$ are the set of the local patterns in training set, which may not generalize to eval set. During finetuning, $\alpha_i$ for $i \in Pa_{train}$ increases. While increased $\alpha_i$ for $i \in Pa_d$ contributes to learning knowledge in domain $d$, higher $\alpha_i$ for $i \in Pa_{train}-Pa_d$ harms the generalization of the model, leading to overfitting. When the effect of overfitting is much bigger that better higher $\alpha_i$ for real patterns, training process ends, leaving these $\alpha_i$ lower than expected. As a consequence, patterns not in $d$ get relatively higher importance factor, making the model to generate out of domain samples.

